Visually grounded models of spoken language: A survey of datasets, architectures and evaluation techniques

This survey provides an overview of the evolution of visually grounded models of spoken language over the last 20 years. Such models are inspired by the observation that when children pick up a language, they rely on a wide range of indirect and noisy clues, crucially including signals from the visual modality co-occurring with spoken utterances. Several fields have made important contributions to this approach to modeling or mimicking the process of learning language: Machine Learning, Natural Language and Speech Processing, Computer Vision and Cognitive Science. The current paper brings together these contributions in order to provide a useful introduction and overview for practitioners in all these areas. We discuss the central research questions addressed, the timeline of developments, and the datasets which enabled much of this work. We then summarize the main modeling architectures and offer an exhaustive overview of the evaluation metrics and analysis techniques.

==> notes.tex <==
% To fix

Spoken moments work uses ASR.

% To add
 Räsänen, O. & Khorrami, K. (2019), A computational Model of Early Language Acquisi-
 tion from Audiovisual Experiences of Young Infants, in ‘Interspeech
 2019, 20st Annual Conference of the International Speech Communication
 Association, Graz, Austria, 15-19 September 2019’, pp. 3594–3598.
 URL: https: // doi. org/ 10. 21437/ interspeech. 2019-1523

Krishnamohan, V., Soman, A., Gupta, A. & Ganapathy, S. (2020), Audiovisual Correspon-
dence Learning in Humans and Machines, in ‘Interspeech 2020, 21st Annual Conference
of the International Speech Communication Association, Virtual Event, Shanghai, China,
25-29 October 2020’, pp. 4462–4466.
URL: http: // dx. doi. org/ 10. 21437/ Interspeech. 2020-2674

Drexler, J. & Glass, J. (2017), Analysis of Audio-Visual Features for Unsupervised Speech
Recognition, in ‘Proc. GLU 2017 International Workshop on Grounding Language Un-
derstanding’, pp. 57–61.
URL: http: // dx. doi. org/ 10. 21437/ GLU. 2017-12

\appendix
\section{List of papers}
\paragraph{Roy}
\citet{roy2000grounded,roy2000learning,roy2001situation,roy2002learning,roypentland2002learning,roy2002grounding,roy2002trainable,roy2002towards,mukherjee2003visual,gorniak2003visually,roy2003grounded,roy2005towards,roy2005grounding}
\paragraph{Harwath}
\citet{harwath2015deep,harwath2016unsupervised,leidal2017learning,
  harwath-glass-2017-learning,harwath2018learning,harwath2018vision,azuh2019towards,harwath2019towards,boggust2019grounding,
  harwath2020learning,harwath2020jointly,ohishi2020trilingual,hsu2020textfree}

\paragraph{Chrupała}
\citet{gelderloos-chrupala-2016-phonemes,chrupala-etal-2017-representations,
  alishahi-etal-2017-encoding,chrupala-2019-symbolic,chrupala-etal-2019-difficulty,
  chrupala-etal-2020-analyzing,gelderloos-etal-2020-learning,higy-etal-2020-textual,anonymous2021discrete}

\paragraph{Kamper}
\citet{kamper2017visually,kamper2018visually,kamper2019semantic,eloff2019multimodal,
  kamper2019semantic-ieee,nortje2020unsupervised,nortje2020direct,olaleye2020localisation}




\paragraph{Merkx}
\citet{Merkx2019,merkx2019learning,scholten2020learning}


\paragraph{Havard}
\citet{havard2017speech,havard2019word,havard2019models,havard2020catplayinginthesnow}

\paragraph{Others}
\citet{yu2004multimodal,mangin2013learning,mangin2015mca,leidal2018neural,scharenborg2018linguistic,vasudevan2018object,hsu2019transfer,boggust2019grounding,ilharco-etal-2019-large,wang2020show,ohishi2020trilingual,rouditchenko2020avlnet,wang2020dnn,wang2020align,ebert2020visuospatial,shukla2020learning,khorrami_2021}

\section{Notes on papers}
\paragraph{\citet{shukla2020learning}} Also about talking heads but combines with self-supervision.

\paragraph{\citet{hsu2020textfree}} Speech captioning without text as
an intermediate representation, or supervision signal.  Factored into
image-to-unit and unit-to-speech modules. Units discovered via
self-supervision. Assumes speech to be independent of image,
conditional on image (this works for captioning but not in
general?). U2S model uses something called Tacotron-2
(unit->spectrograms) and  WaveGlow (spectrogram->waveform).


\paragraph{\citet{wang2020dnn}} seems like it works with gold phone labels,
although there is this setting {\it concept-to-audio} which doesn't
use it, but does use gold boundaries? Anyway very hard to make sense of.


\paragraph{\citet{eloff2019multimodal}} One-shot learning of
associations of images with spoken labels. Images and labels are
digits (11: oh and zero). They do this via retrieval on the support
(different from training) set. Experiments with Siamese networks to
train unimodal distance metrics. Compare distance metric on raw
features to ``learned'' metric trained on separate bimodal training
data. Mysterious Online semi-hard mining. (F. Schroff,
D. Kalenichenko, and J. Philbin, “Facenet: A unified embedding for
face recognition and clustering,” in Proc. CVPR, 2015.) For each
positive pair, the most difficult negative example $x_n$ satisfying $D(x_a
, x_p ) < D(x_a , x_n )$ is then used. TIDigits corpus, MNIST. Batch
all strategy from (A. Hermans, L. Beyer, and B. Leibe, “In defense of the
triplet loss for person re-identification,” arXiv preprint
arXiv:1703.07737, 2017.) Some stuff with siamese online vs offline
which I don't fully get. Tested speaker invariance.

\paragraph{\citet{ngiam2011multimodal}} ``focus on learning
representations for speech audio which are coupled with videos of the
lips'' so this is in the vein vision for phonetics, not vision for
semantics. Worth pointing out the distinction. Data: digits, letters, timit.

\paragraph{\citet{roy2005towards}} breaking module boundaries; spoken language
understanding system in which visual context primes early stages of
speech processing, resulting in significantly improved speech
recognition and understanding accuracy. The ASR is standard for the
time (supervised via text).

\paragraph{\citet{roy2005grounding}} this is some kind of survey?

\paragraph{\citet{roy2003grounded}} inspired by theories of infant
cognition model learns from acoustic and video input, integrated in an
information theoretic framework: associations. Implemented in real
time robot. tested on child directed speech/images. This also CELL
even though it doesn't cite \citet{roypentland2002learning}. Instead
it refers to Roy's PhD thesis \citet{roy1999learning}. ``model
discovers words by searching for segments of speech which reliably
predict the presence of co-occurring visual categories''
Noise: ``In experiments with infant-directed
speech described in Section IX, the majority of spoken ut-
terances in our corpus contained no direct reference to the
co-occurring visual contex.t''
Pre-trained English phoneme feature extraction. Utterances represented
as arrays of phoneme probabilities (RNN trained on TIMIT, 69\%
accuracy). Segmented into utterances by detecting contiguous speech
(with low silence prob) Speech segment similarity metric based on HMM
likelihood ratio. For vision, color and shape extractors. Multiple
views represent an object. Hard coded invariances. Hand coded
silhouette representations. $X^2$ as a distance metric between object shapes.

\paragraph{\citet{roypentland2002learning}} ``learns to segment speech at word boundaries, form visual categories, and acquire semantically appropriate associations between spoken words and visual categories''

RNN for the speech signal, histograms
of stuff for the visual signal. Memory stores (STM and LTM) integrate
these. ''speech and images are analyzed together to find recurrent
segments of speech in similar visual contexts''. They use thresholds
and MI to filter bad associations out. ``lack of visual input led to
over a 50\% drop in word discovery accuracy''

\paragraph{\citet{roy2003grounded}} ``CELL has been integrated into an
interactive word learning robot that learns to use color and shape
names to interpret and generate two-word descriptive phrases of
objects''

\paragraph{\citet{yu2005role}} ``a system that processes spoken input
paired with visual images of multiple objects combined with the
speaker's eye gaze direction''. speakers recorded narrating stories
based on illustrations - eye tracker tracked gaze. Cross-modal
associative learning similar to CELL (+gaze). Ablations without vision
and without gaze.

\section{Architecture details}
\paragraph{\citet{harwath2016unsupervised}}
\begin{enumerate}
\item Convolution: C=64, W=5, H=40, ReLU
\item Maxpool: W=4, S=2
\item Convolution: C=512, W=25, H=1, ReLU
\item Maxpool: W=4, S=2
\item Convolution: C=1024, W=25, H=1, ReLU
\item Mean/Maxpool over entire caption
\item L2 norm
\end{enumerate}

\paragraph{\citet{harwath-glass-2017-learning}}
\begin{enumerate}
\item Convolution: C=128, W=1, H=40, ReLU
\item Convolution: C=256, W=11, H=1, ReLU
\item Maxpool: W=3, H=1, S=2
\item Convolution: C=512, W=17, H=1, ReLU
\item Maxpool: W=3, H=1, S=2
\item Convolution: C=512, W=17, H=1, ReLU
\item Maxpool: W=3, H=1, S=2
\item Convolution: C=1024, W=17, H=1, ReLU
\item Meanpool over entire caption
\item L2 norm
\end{enumerate}

\paragraph{\citet{chrupala-etal-2020-analyzing}}
\begin{itemize}
\item Convolution1D: C=64, W=6, S=2
\item BidiGRU: H=1024, D=4
\item AttnPool over entire caption H=128
\item L2 norm
\end{itemize}


\paragraph{ResDAVEnet \citet{hsu2019transfer}}
The first layer of the ResDAVEnet audio model is comprised of 128
convolutional units each spanning all frequency channels but only one
temporal frame, with a temporal shift of 1 frame. This is followed by
a ReLU and a BatchNorm layer. The remainder of the network is a se-
quence of 4 residual stacks with channel dimensions 128, 256, 512, and
1024. Each residual stack is comprised of a sequence of two basic
residual blocks (as described in [26]) which share the same overall
channel dimension, with 2-D 3x3 kernels re- placed with 1-D kernels of
length 9. Additionally, the first resid- ual block in each layer in
each stack is applied with a stride of two frames, resulting in an
effective temporal downsampling ratio of 2 4 for the entire network

\begin{itemize}
\item Convolution: C=128, W=1, H=40, S=1, ReLU
\item BatchNorm
\item ResBlock x 2: C=128, S=2
\item ResBlock x 2: C=256, S=2
\item ResBlock x 2: C=512, S=2
\item ResBlock x 2: C=1024, S=2
\end{itemize}

\paragraph{Analysis}
\citet{alishahi-etal-2017-encoding} propose several approaches to
evaluating the encoding of phonological form and apply them to the
model of \citet{chrupala-etal-2017-representations} trained on the
Synthetically Spoken COCO dataset. Overall, they find that phoneme
representations are most salient in lower layers of the architecture,
although do persist even in the top
layers. \citet{chrupala-etal-2020-analyzing} perform a comparative
study of the main approaches to testing for the encoding of phonology
in several conditions and recommend a number of best practices, most
importantly using untrained target models as a baseline and reporting
the outcomes of multiple metrics.
\citet{harwath2020learning} and \citet{anonymous2021discrete} evaluate
discrete representations specifically.

